Capacity Bounds under Imperfect Polarization Tracking

In optical fiber communication, due to the random variation of the environment, the state of polarization (SOP) fluctuates randomly with time leading to distortion and performance degradation. The memory-less SOP fluctuations can be regarded as a two-by-two random unitary matrix. In this paper, for what we believe to be the first time, the capacity of the polarization drift channel under an average power constraint with imperfect channel knowledge is characterized. An achievable information rate (AIR) is derived when imperfect channel knowledge is available and is shown to be highly dependent on the channel estimation technique. It is also shown that a tighter lower bound can be achieved when a unitary estimation of the channel is available. However, the conventional estimation algorithms do not guarantee a unitary channel estimation. Therefore, by considering the unitary constraint of the channel, a data-aided channel estimator based on the Kabsch algorithm is proposed, and its performance is numerically evaluated in terms of AIR. Monte Carlo simulations show that Kabsch outperforms the least-square error algorithm. In particular, with complex, Gaussian inputs and eight pilot symbols per block, Kabsch improves the AIR by 0:2 to 0:35 bits/symbol throughout the range of studied signal-to-noise ratios.

==> TCOM_MF_EA_MK_ Submitted/acronym.tex <==
\DeclareAcronym{SOP}{
short=SOP,
long= state of polarization,
}

\DeclareAcronym{AIR}{
short=AIR,
long= achievable information rate,
}

\DeclareAcronym{DSP}{
short=DSP,
long= digital signal processing,
}

\DeclareAcronym{PMD}{
short=PMD,
long= polarization-mode dispersion,
}

\DeclareAcronym{DOF}{
short=DOF,
long= degrees of freedom,
}

\DeclareAcronym{CMA}{
short=CMA,
long= constant modulus algorithm,
}
\DeclareAcronym{MMA}{
short=MMA,
long= multi-modulus algorithm,
}
\DeclareAcronym{RDE}{
short=RDE,
long= radially directed equalizer,
}

\DeclareAcronym{QAM}{
short=QAM,
long= quadrature amplitude modulation,
}

\DeclareAcronym{LMS}{
short=LMS,
long= least mean square,
}

\DeclareAcronym{LS}{
short=LS,
long= least-square error,
}

\DeclareAcronym{DP}{
short=DP,
long= dual-polarization,
}

\DeclareAcronym{PN}{
short=PN,
long= phase noise,
}

\DeclareAcronym{GN}{
short=GN,
long= Gaussian Noise,
}

\DeclareAcronym{NLI}{
short=NLI,
long= nonlinear impairments,
}

\DeclareAcronym{MIMO}{
short=MIMO,
long=  multiple-input multiple-output,
}

\DeclareAcronym{SNR}{
short=SNR,
long= signal-to-noise ratio,
}

\DeclareAcronym{MI}{
short=MI,
long= mutual information,
}

\DeclareAcronym{pdf}{
short=pdf,
long= probability density function,
}

\DeclareAcronym{AWGN}{
short=AWGN,
long= additive white Gaussian noise,
}

\DeclareAcronym{ASE}{
short=ASE,
long= amplified spontaneous emission,
}

\DeclareAcronym{QPSK}{
short=QPSK,
long= quadrature phase-shift keying,
}
%\ac,
%\acf
%\Ac
%\acp
%\acfp
